Limits on the nuclearite flux using the ANTARES neutrino telescope

In this work, a search for nuclearites of strange quark matter by using nine years of ANTARES data taken in the period 2009-2017 is presented. The passage through matter of these particles is simulated %according to the model of de R\'{u}jula and Glashow taking into account a detailed description of the detector response to nuclearites and of the data acquisition conditions. A down-going flux of cosmic nuclearites with Galactic velocities ($\beta = 10^{-3}$) was considered for this study. The mass threshold for detecting these particles at the detector level is \mbox{ $4 \times 10^{13}$ GeV/c$^{2}$}. Upper limits on the nuclearite flux for masses up to $10^{17}$ GeV/c$^{2}$ at the level of $\sim 5 \times 10^{-17}$ cm$^{-2}$ s$^{-1}$ sr$^{-1}$ are obtained. These are the first upper limits on nuclearites established with a neutrino telescope and the most stringent ever set for Galactic velocities.

==> other/author_list.tex <==
%\documentclass{elsarticle}
%\journal{}
%\begin{document}
%\begin{frontmatter}
%\title{ANTARES collaboration}
\author[IPHC,UHA]{A.~Albert}
\author[IFIC]{S.~Alves}
\author[UPC]{M.~Andr\'e}
\author[UPV]{M.~Ardid}
\author[UPV]{S.~Ardid}
\author[CPPM]{J.-J.~Aubert}
\author[APC]{J.~Aublin}
\author[APC]{B.~Baret}
\author[LAM]{S.~Basa}
\author[CNESTEN]{B.~Belhorma}
\author[APC,Rabat]{M.~Bendahman}
\author[Bologna,Bologna-UNI]{F.~Benfenati}
\author[CPPM]{V.~Bertin}
\author[LNS]{S.~Biagi}
\author[Erlangen]{M.~Bissinger}
\author[Rabat]{J.~Boumaaza}
\author[LPMR]{M.~Bouta}
\author[NIKHEF]{M.C.~Bouwhuis}
\author[ISS]{H.~Br\^{a}nza\c{s}}
\author[NIKHEF,UvA]{R.~Bruijn}
\author[CPPM]{J.~Brunner}
\author[CPPM]{J.~Busto}
\author[Genova]{B.~Caiffi}
\author[IFIC]{D.~Calvo}
\author[Roma,Roma-UNI]{A.~Capone}
\author[ISS]{L.~Caramete}
\author[CPPM]{J.~Carr}
\author[IFIC]{V.~Carretero}
\author[Roma,Roma-UNI]{S.~Celli}
\author[Marrakech]{M.~Chabab}
\author[APC]{T. N.~Chau}
\author[Rabat]{R.~Cherkaoui El Moursli}
\author[Bologna]{T.~Chiarusi}
\author[Bari]{M.~Circella}
\author[APC]{A.~Coleiro}
\author[LNS]{R.~Coniglione}
\author[CPPM]{P.~Coyle}
\author[APC]{A.~Creusot}
\author[UGR-CITIC]{A.~F.~D\'\i{}az}
\author[APC]{G.~de~Wasseige}
\author[CPPM]{B.~De~Martino}
\author[LNS]{C.~Distefano}
\author[Roma,Roma-UNI]{I.~Di~Palma}
\author[NIKHEF,UvA]{A.~Domi}
\author[APC,UPS]{C.~Donzaud}
\author[CPPM]{D.~Dornic}
\author[IPHC,UHA]{D.~Drouhin}
\author[Erlangen]{T.~Eberl}
\author[NIKHEF]{T.~van~Eeden}
\author[NIKHEF]{D.~van~Eijk}
\author[Rabat]{N.~El~Khayati}
\author[CPPM]{A.~Enzenh\"ofer}
\author[Roma,Roma-UNI]{P.~Fermani}
\author[LNS]{G.~Ferrara}
\author[Bologna,Bologna-UNI]{F.~Filippini}
\author[Salerno-UNI]{L.~Fusco}
\author[UPV]{J.~Garc\'\i{}a-M\'endez}
\author[Clermont-Ferrand,APC]{P.~Gay}
\author[LSIS]{H.~Glotin}
\author[IFIC]{R.~Gozzini}
\author[NIKHEF]{R.~Gracia~Ruiz}
\author[Erlangen]{K.~Graf}
\author[Genova,Genova-UNI]{C.~Guidi}
\author[Erlangen]{S.~Hallmann}
\author[NIOZ]{H.~van~Haren}
\author[NIKHEF]{A.J.~Heijboer}
\author[GEOAZUR]{Y.~Hello}
\author[IFIC]{J.J. ~Hern\'andez-Rey}
\author[Erlangen]{J.~H\"o{\ss}l}
\author[Erlangen]{J.~Hofest\"adt}
\author[CPPM]{F.~Huang}
\author[Bologna,Bologna-UNI]{G.~Illuminati}
\author[Curtin]{C.~W.~James}
\author[NIKHEF]{B.~Jisse-Jung}
\author[NIKHEF,Leiden]{M. de~Jong}
\author[NIKHEF,UvA]{P. de~Jong}
\author[Wuerzburg]{M.~Kadler}
\author[Erlangen]{O.~Kalekin}
\author[Erlangen]{U.~Katz}
\author[APC]{A.~Kouchner}
\author[Bamberg]{I.~Kreykenbohm}
\author[Genova]{V.~Kulikovskiy}
\author[Erlangen]{R.~Lahmann}
\author[APC]{M.~Lamoureux}
\author[APC]{R.~Le~Breton}
\author[COM]{D. ~Lef\`evre}
\author[Catania]{E.~Leonora}
\author[Bologna,Bologna-UNI]{G.~Levi}
\author[CPPM]{S.~Le~Stum}
\author[UGR-CAFPE]{D.~Lopez-Coto}
\author[IRFU/SPP,APC]{S.~Loucatos}
\author[APC]{L.~Maderer}
\author[IFIC]{J.~Manczak}
\author[LAM]{M.~Marcelin}
\author[Bologna,Bologna-UNI]{A.~Margiotta}
\author[Napoli]{A.~Marinelli}
\author[UPV]{J.A.~Mart\'inez-Mora}
\author[NIKHEF,UvA]{K.~Melis}
\author[Napoli]{P.~Migliozzi}
\author[LPMR]{A.~Moussa}
\author[NIKHEF]{R.~Muller}
\author[NIKHEF]{L.~Nauta}
\author[UGR-CAFPE]{S.~Navas}
\author[LAM]{E.~Nezri}
\author[NIKHEF]{B.~\'O~Fearraigh}
\author[ISS]{A.~P\u{a}un}
\author[ISS]{G.E.~P\u{a}v\u{a}la\c{s}}
\author[Bologna,Roma-Museo,CNAF]{C.~Pellegrino}
\author[CPPM]{M.~Perrin-Terrin}
\author[NIKHEF]{V.~Pestel}
\author[LNS]{P.~Piattelli}
\author[IFIC]{C.~Pieterse}
\author[UPV]{C.~Poir\`e}
\author[ISS]{V.~Popa}
\author[IPHC]{T.~Pradier}
\author[Catania]{N.~Randazzo}
\author[IFIC]{D.~Real}
\author[Erlangen]{S.~Reck}
\author[LNS]{G.~Riccobene}
\author[Genova,Genova-UNI]{A.~Romanov}
\author[IFIC,Bari]{A.~S\'anchez-Losa}
\author[IFIC]{F.~Salesa~Greus}
\author[NIKHEF,Leiden]{D. F. E.~Samtleben}
\author[Genova,Genova-UNI]{M.~Sanguineti}
\author[LNS]{P.~Sapienza}
\author[Erlangen]{J.~Schnabel}
\author[Erlangen]{J.~Schumann}
\author[IRFU/SPP]{F.~Sch\"ussler}
\author[NIKHEF]{J.~Seneca}
\author[Bologna,Bologna-UNI]{M.~Spurio}
\author[IRFU/SPP]{Th.~Stolarczyk}
\author[Genova,Genova-UNI]{M.~Taiuti}
\author[Rabat,BenGuerir]{Y.~Tayalati}
\author[Curtin]{S.J.~Tingay}
\author[IRFU/SPP,APC]{B.~Vallage}
\author[APC,IUF]{V.~Van~Elewyck}
\author[Bologna,Bologna-UNI,APC]{F.~Versari}
\author[LNS]{S.~Viola}
\author[Napoli,Napoli-UNI]{D.~Vivolo}
\author[Bamberg]{J.~Wilms}
\author[Genova]{S.~Zavatarelli}
\author[Roma,Roma-UNI]{A.~Zegarelli}
\author[IFIC]{J.D.~Zornoza}
\author[IFIC]{J.~Z\'u\~{n}iga}


\address[IPHC]{\scriptsize{Universit\'e de Strasbourg, CNRS,  IPHC UMR 7178, F-67000 Strasbourg, France}}
\address[UHA]{\scriptsize Universit\'e de Haute Alsace, F-68100 Mulhouse, France}
\address[IFIC]{\scriptsize{IFIC - Instituto de F\'isica Corpuscular (CSIC - Universitat de Val\`encia) c/ Catedr\'atico Jos\'e Beltr\'an, 2 E-46980 Paterna, Valencia, Spain}}
\address[UPC]{\scriptsize{Technical University of Catalonia, Laboratory of Applied Bioacoustics, Rambla Exposici\'o, 08800 Vilanova i la Geltr\'u, Barcelona, Spain}}
\address[UPV]{\scriptsize{Institut d'Investigaci\'o per a la Gesti\'o Integrada de les Zones Costaneres (IGIC) - Universitat Polit\`ecnica de Val\`encia. C/  Paranimf 1, 46730 Gandia, Spain}}
\address[CPPM]{\scriptsize{Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}}
\address[APC]{\scriptsize{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}}
\address[LAM]{\scriptsize{Aix Marseille Univ, CNRS, CNES, LAM, Marseille, France }}
\address[CNESTEN]{\scriptsize{National Center for Energy Sciences and Nuclear Techniques, B.P.1382, R. P.10001 Rabat, Morocco}}
\address[Rabat]{\scriptsize{Mohammed V University in Rabat, Faculty of Sciences, 4 av. Ibn Battouta, B.P. 1014, R.P. 10000
Rabat, Morocco}}
%\address[RabatNew]{\scriptsize{Mohammed V University in Rabat}}
\address[BenGuerir]{\scriptsize{Institute of Applied Physics, Mohammed VI Polytechnic University, Lot 660, Hay Moulay Rachid Ben Guerir, 43150, Morocco.}}
\address[Bologna]{\scriptsize{INFN - Sezione di Bologna, Viale Berti-Pichat 6/2, 40127 Bologna, Italy}}
\address[Bologna-UNI]{\scriptsize{Dipartimento di Fisica e Astronomia dell'Universit\`a, Viale Berti Pichat 6/2, 40127 Bologna, Italy}}
\address[LNS]{\scriptsize{INFN - Laboratori Nazionali del Sud (LNS), Via S. Sofia 62, 95123 Catania, Italy}}
\address[Erlangen]{\scriptsize{Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, Erwin-Rommel-Str. 1, 91058 Erlangen, Germany}}
\address[LPMR]{\scriptsize{University Mohammed I, Laboratory of Physics of Matter and Radiations, B.P.717, Oujda 6000, Morocco}}
\address[NIKHEF]{\scriptsize{Nikhef, Science Park,  Amsterdam, The Netherlands}}
\address[ISS]{\scriptsize{Institute of Space Science, RO-077125 Bucharest, M\u{a}gurele, Romania}}
\address[UvA]{\scriptsize{Universiteit van Amsterdam, Instituut voor Hoge-Energie Fysica, Science Park 105, 1098 XG Amsterdam, The Netherlands}}
\address[Genova]{\scriptsize{INFN - Sezione di Genova, Via Dodecaneso 33, 16146 Genova, Italy}}
\address[Roma]{\scriptsize{INFN - Sezione di Roma, P.le Aldo Moro 2, 00185 Roma, Italy}}
\address[Roma-UNI]{\scriptsize{Dipartimento di Fisica dell'Universit\`a La Sapienza, P.le Aldo Moro 2, 00185 Roma, Italy}}
\address[Marrakech]{\scriptsize{LPHEA, Faculty of Science - Semlali, Cadi Ayyad University, P.O.B. 2390, Marrakech, Morocco.}}
\address[Bari]{\scriptsize{INFN - Sezione di Bari, Via E. Orabona 4, 70126 Bari, Italy}}
\address[UGR-CITIC]{\scriptsize{Department of Computer Architecture and Technology/CITIC, University of Granada, 18071 Granada, Spain}}
\address[UPS]{\scriptsize{Universit\'e Paris-Sud, 91405 Orsay Cedex, France}}
\address[Salerno-UNI]{\scriptsize{Universit\`a di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Fisica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy}}
\address[Clermont-Ferrand]{\scriptsize{Laboratoire de Physique Corpusculaire, Clermont Universit\'e, Universit\'e Blaise Pascal, CNRS/IN2P3, BP 10448, F-63000 Clermont-Ferrand, France}}
\address[LSIS]{\scriptsize{LIS, UMR Universit\'e de Toulon, Aix Marseille Universit\'e, CNRS, 83041 Toulon, France}}
\address[Genova-UNI]{\scriptsize{Dipartimento di Fisica dell'Universit\`a, Via Dodecaneso 33, 16146 Genova, Italy}}
\address[NIOZ]{\scriptsize{Royal Netherlands Institute for Sea Research (NIOZ), Landsdiep 4, 1797 SZ 't Horntje (Texel), the Netherlands}}
\address[GEOAZUR]{\scriptsize{G\'eoazur, UCA, CNRS, IRD, Observatoire de la C\^ote d'Azur, Sophia Antipolis, France}}
\address[Curtin]{\scriptsize{International Centre for Radio Astronomy Research - Curtin University, Bentley, WA 6102, Australia}}
\address[Leiden]{\scriptsize{Huygens-Kamerlingh Onnes Laboratorium, Universiteit Leiden, The Netherlands}}
\address[Wuerzburg]{\scriptsize{Institut f\"ur Theoretische Physik und Astrophysik, Universit\"at W\"urzburg, Emil-Fischer Str. 31, 97074 W\"urzburg, Germany}}
\address[Bamberg]{\scriptsize{Dr. Remeis-Sternwarte and ECAP, Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg,  Sternwartstr. 7, 96049 Bamberg, Germany}}
\address[COM]{\scriptsize{Mediterranean Institute of Oceanography (MIO), Aix-Marseille University, 13288, Marseille, Cedex 9, France; Universit\'e du Sud Toulon-Var,  CNRS-INSU/IRD UM 110, 83957, La Garde Cedex, France}}
\address[Catania]{\scriptsize{INFN - Sezione di Catania, Via S. Sofia 64, 95123 Catania, Italy}}
\address[UGR-CAFPE]{\scriptsize{Dpto. de F\'\i{}sica Te\'orica y del Cosmos \& C.A.F.P.E., University of Granada, 18071 Granada, Spain}}
\address[IRFU/SPP]{\scriptsize{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}}
\address[Napoli]{\scriptsize{INFN - Sezione di Napoli, Via Cintia 80126 Napoli, Italy}}
\address[Roma-Museo]{\scriptsize{Museo Storico della Fisica e Centro Studi e Ricerche Enrico Fermi, Piazza del Viminale 1, 00184, Roma}}
\address[CNAF]{\scriptsize{INFN - CNAF, Viale C. Berti Pichat 6/2, 40127, Bologna}}
\address[IUF]{\scriptsize{Institut Universitaire de France, 75005 Paris, France}}
\address[Napoli-UNI]{\scriptsize{Dipartimento di Fisica dell'Universit\`a Federico II di Napoli, Via Cintia 80126, Napoli, Italy}}
%\end{frontmatter}
%\end{document}

